SoTTA: Robust Test-Time Adaptation on Noisy Data Streams

Test-time adaptation (TTA) aims to address distributional shifts between training and testing data using only unlabeled test data streams for continual model adaptation. However, most TTA methods assume benign test streams, while test samples could be unexpectedly diverse in the wild. For instance, an unseen object or noise could appear in autonomous driving. This leads to a new threat to existing TTA algorithms; we found that prior TTA algorithms suffer from those noisy test samples as they blindly adapt to incoming samples. To address this problem, we present Screening-out Test-Time Adaptation (SoTTA), a novel TTA algorithm that is robust to noisy samples. The key enabler of SoTTA is two-fold: (i) input-wise robustness via high-confidence uniform-class sampling that effectively filters out the impact of noisy samples and (ii) parameter-wise robustness via entropy-sharpness minimization that improves the robustness of model parameters against large gradients from noisy samples. Our evaluation with standard TTA benchmarks with various noisy scenarios shows that our method outperforms state-of-the-art TTA methods under the presence of noisy samples and achieves comparable accuracy to those methods without noisy samples. The source code is available at https://github.com/taeckyung/SoTTA .

==> rebuttal.tex <==
\clearpage
\pagenumbering{gobble}

\begin{center}
    {\bf {\LARGE Rebuttal}} \\
    \vspace{0.15in}
    {\bf {\Large \system{}: Robust Test-Time Adaptation on Noisy Data Streams}} \\

\vspace{1.5cm}
   
\end{center}


\begin{figure}[t!]
\centering
\begin{minipage}{\textwidth}
\centering
\begin{wrapfigure}{!t}{0.95\textwidth}
    \centering
    \begin{subfigure}[!t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/plot_hyperparam_c0.pdf}
    \caption{Effect of hyperparameter $C_0$.}
    \end{subfigure}
    \hspace{-0.1cm}
    \begin{subfigure}[!t]{0.49\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/plot_hyperparam_m.pdf}
    \caption{Effect of hyperparameter $m$.}
    % \vspace{-0.3cm}
    \end{subfigure}
    \caption{Effect of hyperparameters on the model accuracy on CIFAR10-C with ResNet-18 for 15 types of corruptions under five scenarios: Benign, Near, Far, Attack, and Noise. Averaged over three different random seeds.}
    % \hfill
\end{wrapfigure}
\end{minipage}
\end{figure}

% \begin{table}[h]
% \centering
% \caption{Average True Positive Rate (\%) and Average True Negative Rate (\%) of ODIN~\cite{odin} algorithm with optimal threshold. Average Classification accuracy (\%) of ODIN+TTA on CIFAR10-C with ResNet-18. \textbf{Bold} numbers are the accuracy with improvement from normal TTAs.}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{llccccccccccccccc
% >{\columncolor[HTML]{EDEEFF}}c }
% \Xhline{2\arrayrulewidth}
% \addlinespace[0.08cm] 
%  &  & \multicolumn{3}{c}{Benign} & \multicolumn{3}{c}{Near} & \multicolumn{3}{c}{Far} & \multicolumn{3}{c}{Attack} & \multicolumn{3}{c}{Noise} \\
% \addlinespace[0.00cm] 
% \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} \cmidrule(lr){15-17}
% \addlinespace[0.00cm] 
%  & Method & TPR/TNR & w/o ODIN & with ODIN & TPR/TNR & w/o ODIN & with ODIN & TPR/TNR & w/o ODIN & with ODIN & TPR/TNR & w/o ODIN & with ODIN & TPR/TNR & w/o ODIN & with ODIN \\ \hline
% \addlinespace[0.1cm] 
%  & Source & 100.0/0.0 & 57.45 & 57.45 & 100.0/0.0  & 57.45 & 57.45 & 100.0/0.0   & 57.45 & 57.45 & 100.0/0.0  & 57.45 & 57.45 & 100.0/0.0   & 57.45 & 57.45 \\
%  & BN stats~\cite{bnstats} & 100.0/0.0 & 78.12         & 78.12 & 100.0/0.0  & 76.49         & 76.49 & 96.04/30.05 & 75.44         & \textbf{75.93} & 100.0/0.0  & 55.84         & 55.84 & 83.4/56.69  & 55.89         & \textbf{56.67} \\
%  & PL~\cite{pl} & 99.53/0.0 & 78.36         & \textbf{78.81} & 99.86/0.29 & 73.03 & \textbf{74.26} & 98.71/4.73  & 71.31         & \textbf{71.61} & 99.86/0.28 & 66.45         & \textbf{66.49} & 100.0/0.0   & 52.15         & 52.15  \\
%  & TENT~\cite{tent} & 100.0/0.0 & 81.46         & 81.46 & 98.56/3.21 & 74.50         & \textbf{76.05} & 99.70/0.69  & 73.49         & \textbf{74.72} & 99.62/0.43 & 68.98         & \textbf{69.10} & 78.98/68.47 & 54.40         & \textbf{56.20} \\
%  & LAME~\cite{lame} & 100.0/0.0 & 56.12         & 56.12 & 100.0/0.0  & 56.70 & 56.70  & 99.74/1.70   & 55.73         & \textbf{55.74} & 100.0/0.0  & 56.15         & 56.15 & 95.61/72.88 & 54.89         & \textbf{55.23} \\
%  & CoTTA~\cite{cotta} & 100.0/0.0 & 82.15 & 82.15 & 100.0/0.0 & 78.17 & 78.17 & 100.0/0.0 & 73.58 & 73.58 & 100.0/0.0 & 69.60 & 69.60 & 77.06/86.29 & 57.78 & \textbf{62.04} \\
% & SAR~\cite{sar} & 100.0/0.0 & 78.41 & 78.41 & 100.0/0.0 & 77.51 & 77.51 & 98.91/10.62 & 75.68 & \textbf{76.03} & 100.0/0.0 & 56.20 & 56.20 & 100.0/0.0 & 58.71 & 58.71 \\
%  & RoTTA~\cite{rotta} & 100.0/0.0 & 75.29 & 75.29 & 100.0/0.0 & 77.46 & 77.46 & 100.0/0.0 & 76.98 & 76.98 & 100.0/0.0 & 78.40 & 78.40 & 100.0/0.0 & 73.44 & 73.44 \\
% &  SoTTA & 100.0/0.0 & 82.07 & 82.07 & 100.0/0.0 & 81.58 & 81.58 & 99.90/6.61 & 81.74 & \textbf{82.03} & 100.0/0.0 & 84.50 & 84.50 & 100.0/0.0 & 81.46 & 81.46 \\
% \Xhline{2\arrayrulewidth}
% \end{tabular}%
% }
% \end{table}


\begin{figure}[!b]
\centering

\begin{minipage}{\textwidth}
\centering
\vspace{-4.5cm}
\begin{table}[H]
\centering
\caption{Average classification accuracy (\%) of ODIN+TTA on CIFAR10-C with ResNet-18. \textbf{Bold} numbers are the accuracy with improvement from normal TTAs. Averaged over three different random seeds.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccccccc}
\Xhline{2\arrayrulewidth}
\addlinespace[0.08cm] 
  & \multicolumn{2}{c}{Benign} & \multicolumn{2}{c}{Near} & \multicolumn{2}{c}{Far} & \multicolumn{2}{c}{Attack} & \multicolumn{2}{c}{Noise} \\
\addlinespace[0.00cm] 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
\addlinespace[0.00cm] 
Method & w/o ODIN & with ODIN & w/o ODIN & with ODIN & w/o ODIN & with ODIN & w/o ODIN & with ODIN & w/o ODIN & with ODIN  \\ \hline
\addlinespace[0.1cm] 
Source & 57.45 & 57.45 & 57.45 & 57.45 & 57.45 & 57.45 & 57.45 & 57.45 & 57.45 & 57.45 \\
BN stats~\cite{bnstats} & 78.12 & 78.12 & 76.49 & 76.49 & 75.44 & \textbf{75.93} & 55.84 & 55.84 & 55.89 & \textbf{56.67} \\
PL~\cite{pl} & 78.36 & \textbf{78.81} & 73.03 & \textbf{74.26} & 71.31 & \textbf{71.61} & 66.45 & \textbf{66.49} & 52.15 & 52.15 \\
TENT~\cite{tent} & 81.46 & 81.46 & 74.50 & \textbf{76.05} & 73.49 & \textbf{74.72} & 68.98 & \textbf{69.10} & 54.40 & \textbf{56.20} \\
LAME~\cite{lame} & 56.12 & 56.12 & 56.70 & 56.70 & 55.73 & \textbf{55.74} & 56.15 & 56.15 & 54.89 & \textbf{55.23} \\
CoTTA~\cite{cotta} & 82.15 & 82.15 & 78.17 & 78.17 & 73.58 & 73.58 & 69.60 & 69.60 & 57.78 & \textbf{62.04} \\
SAR~\cite{sar} & 78.41 & 78.41 & 77.51 & 77.51 & 75.68 & \textbf{76.03} & 56.20 & 56.20 & 58.71 & 58.71 \\
RoTTA~\cite{rotta} & 75.29 & 75.29 & 77.46 & 77.46 & 76.98 & 76.98 & 78.40 & 78.40 & 73.44 & 73.44 \\
SoTTA (ours) & 82.07 & 82.07 & 81.58 & 81.58 & 81.74 & \textbf{82.03} & 84.50 & 84.50 & 81.46 & 81.46 \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\end{table}
\end{minipage}%


\begin{minipage}{1.0\textwidth}
\centering
\begin{subfigure}[t]{0.8\linewidth}
\centering
\vspace{1.0cm}
\includegraphics[width=\linewidth]{fig/OOD_th.pdf}
% \caption{ODIN at different threshold values on TENT}
\end{subfigure}

\caption{Effect of OOD threshold $\delta$ on classification accuracy (\%) of ODIN+TENT on CIFAR10-C with ResNet-18. Averaged over three different random seeds.}
\end{minipage}
\end{figure}



\clearpage
